Finding path and cycle counting formulae in graphs with Deep Reinforcement Learning

This paper presents Grammar Reinforcement Learning (GRL), a reinforcement learning algorithm that uses Monte Carlo Tree Search (MCTS) and a transformer architecture that models a Pushdown Automaton (PDA) within a context-free grammar (CFG) framework. Taking as use case the problem of efficiently counting paths and cycles in graphs, a key challenge in network analysis, computer science, biology, and social sciences, GRL discovers new matrix-based formulas for path/cycle counting that improve computational efficiency by factors of two to six w.r.t state-of-the-art approaches. Our contributions include: (i) a framework for generating gramformers that operate within a CFG, (ii) the development of GRL for optimizing formulas within grammatical structures, and (iii) the discovery of novel formulas for graph substructure counting, leading to significant computational improvements.

==> data/EXPQM12.tex <==
PPGN,G$^2$N$^2$
0.231,\textbf{0.102}
0.382,\textbf{0.196}
{0.00276},\textbf{0.0021}
{0.00287},\textbf{0.00211}
{0.0029},\textbf{0.00287}
16.07,\textbf{1.19}
{0.00064},\textbf{0.0000151}
{0.234},\textbf{0.0502}
{0.234},\textbf{0.0503}
{0.229},\textbf{0.0503}
{0.238},\textbf{0.0504}
0.184,\textbf{0.0707}
131 s, 57 s

==> data/EXPQM9GMNreduct12.tex <==
Target,PPGN,G$^2$N$^2$(16),G$^2$N$^2$(32)
$\mu$,0.231,\textbf{0.127},\textbf{0.102}
$\alpha$,0.382,\textbf{0.268},\textbf{0.196}
$\epsilon_{\mathrm{homo}}$,{0.00276},\textbf{0.00268},{0.0021}
$\epsilon_{\mathrm{lumo}}$,{0.00287},\textbf{0.00268},\textbf{0.00211}
$\Delta\epsilon$,{0.0029},{0.00369},\textbf{0.00287}
$R^2$,16.07,\textbf{1.48},\textbf{1.19}
ZPVE,{0.00064},\textbf{0.000203},\textbf{0.0000151}
$U_0$,{0.234},\textbf{0.0745},\textbf{0.0502}
$U$,{0.234},\textbf{0.0744},\textbf{0.0503}
$H$,{0.229},\textbf{0.0746},\textbf{0.0503}
$G$,{0.238},\textbf{0.0744},\textbf{0.0504}
$C_v$,0.184,\textbf{0.0904},\textbf{0.0707}
T $/$ ep,131 s,27 s, 57 s

==> data/EXPQM9reduct12full.tex <==
Target,PPGN,G$^2$N$^2$(16),G$^2$N$^2$(32),G$^2$N$^2$(64)
$\mu$,0.231,\textbf{0.127},\textbf{0.102},\textbf{0.0703}
$\alpha$,0.382,\textbf{0.268},\textbf{0.196},\textbf{0.127}
$\epsilon_{\mathrm{homo}}$,{0.00276},\textbf{0.00268},{0.0021},\textbf{0.00172}
$\epsilon_{\mathrm{lumo}}$,{0.00287},\textbf{0.00268},\textbf{0.00211},\textbf{0.00153}
$\Delta\epsilon$,{0.0029},{0.00369},\textbf{0.00287},\textbf{0.00253}
$R^2$,16.07,\textbf{1.48},\textbf{1.19},\textbf{0.342}
ZPVE,{0.00064},\textbf{0.000203},\textbf{0.0000151},\textbf{0.0000951}
$U_0$,{0.234},\textbf{0.0745},\textbf{0.0502},\textbf{0.0169}
$U$,{0.234},\textbf{0.0744},\textbf{0.0503},\textbf{0.0162}
$H$,{0.229},\textbf{0.0746},\textbf{0.0503},\textbf{0.0176}
$G$,{0.238},\textbf{0.0744},\textbf{0.0504},\textbf{0.0214}
$C_v$,0.184,\textbf{0.0904},\textbf{0.0707},\textbf{0.0429}
Time $/$ epoch,131 s,27 s, 57 s, 102 s

==> section/section1o.tex <==
\section{Introduction}\label{sec: 1}



Paths and cycles are fundamental structures in graph theory, playing a crucial role in various fields such as network analysis, computer science, biology, and social sciences. The ability to efficiently count and enumerate paths and cycles of various lengths is crucial for understanding graph connectivity, redundancy, and robustness, and forms the basis for many graph algorithms used in real-world applications.

In the early 1970s, \cite{harary1971number} introduced algorithms to enumerate cycles of length up to five in a graph. Building on this, two decades later, \cite{alon1997finding} developed and refined algorithms capable of counting cycles of length up to seven. With minor modifications, these algorithms can also be adapted to count cycles at the node level. In a subsequent contribution, \cite{voropaev2012number} established a relationship between the counting of $l$-cycles at the edge level and the counting of $(l-1)$-paths at the edge level via a simple formula. By deriving explicit formulas for counting paths of length up to six at the edge level, they were able to count cycles of length up to seven. More recently, \cite{jokic2022number} rediscovered the formulas for paths of length up to four from \cite{voropaev2012number}. In contrast, \cite{giscard2019general} proposed an algorithm to count cycles and paths of arbitrary lengths, though they acknowledge that their method is slower than those of \cite{alon1997finding} and \cite{voropaev2012number}. Specifically, since these algorithms are based on matrix multiplication, their computational complexity is $\grandO{n^3}$, where $n$ is the number of nodes. As noted by \cite{giscard2019general}, these matrix-based approaches remain the most efficient known methods for counting paths and cycles of lengths up to six and seven, respectively. This leads to a significant open question: Is it possible to design a deep learning-based algorithm capable of discovering more efficient formulas for counting paths at the edge level?

%Graph Neural Networks (GNNs) have recently emerged as powerful tools for processing and analyzing graph-structured data, offering new approaches to the challenges of substructure counting. However, traditional Message Passing Neural Networks (MPNNs) \citep{kipf2016semi,xu2018powerful} are limited in their expressive power, being constrained by the first-order Weisfeiler-Lehman ($\WL 1$) test, a well-known method in graph theory for graph isomorphism testing. To overcome these limitations and capture more complex graph substructures, novel models have been developed that surpass the expressiveness of $\WL 1$. Some of these models emulate the $\WL 3$ test, which involves higher-dimensional color refinements and provides greater discriminative power for graph isomorphism tasks \citep{morris2019wl,maron2018invariant,maron2019provably}. Other approaches have introduced strategies that apply GNNs to subgraphs constructed by specific policies, thereby capturing more intricate structural patterns within the graph \citep{bevilacqua2021equivariant,frasca2022understanding,huang2022boosting}. Additional models enhance expressiveness by incorporating subgraph counting mechanisms, enabling the network to recognize and utilize various subgraph structures \citep{huang2021short,bouritsas2022improving}. Furthermore, techniques from formal language theory have been employed to enhance the expressive power of GNNs by using grammatical structures to encode and process graph data more effectively \citep{balcilarexpresspower,piquenot2024grammatical}. Despite studies demonstrating the ability of GNNs to count substructures at the graph or node level \citep{chen2020can,frasca2022understanding}, the inherent lack of interpretability in GNNs prevents the derivation of explicit algorithms or formulas for substructure counting. This raises an important question: Is it possible to develop an algorithm capable of discovering formulas for counting paths at the edge level?

Recently, \cite{Geerts} established a connection between the third-order Weisfeiler-Leman test ($\WL 3$) and a fragment of the matrix language MATLANG \citep{matlang}, characterized by the operations $\cur L_3 := \{ \cdot, \transpose, \mathrm{diag}, \onevector, \odot \}$. They demonstrated that formulas within this fragment, when applied to adjacency matrices, distinguish the same pairs of graphs as $\WL 3$. Building on these insights, \cite{piquenot2024grammatical} introduced a context-free grammar (CFG) for $\WL 3$, a generative framework that notably includes all the formulas identified by \cite{voropaev2012number}. In our pursuit of discovering edge-level path-counting formulas, we initially set out to develop an algorithm capable of identifying the formulas introduced by \cite{voropaev2012number} within the context of this CFG. Unexpectedly, our algorithm not only recovered the original formulas but also discovered new ones that significantly enhance computational efficiency, reducing the computation time by a factor of two to six.

%\cite{voropaev2012number} introduced explicit matrix formulas for counting paths of length up to six at the edge level within graphs. The substructure counting capabilities of the $\WL 3$ test were investigated at both the graph and node levels by \cite{furer2017combinatorial} and \cite{arvind2020weisfeiler}, revealing its inability to count cycles longer than eight. More recently, \cite{Geerts} established a connection between $\WL 3$ and a fragment of the matrix language MATLANG \citep{matlang}, defined by the set of operations $\cur L_3 := { \cdot,\transpose, \mathrm{diag}, \onevector, \odot }$. They demonstrated that sentences in this fragment, when applied to adjacency matrices, separate the same pairs of graphs as $\WL 3$. Building on this work, \cite{piquenot2024grammatical} developed a context-free grammar (CFG) for $\WL 3$, which notably encompasses all the formulas identified by \cite{voropaev2012number}. To address the question of discovering edge-level path-counting formulas, our original objective was to develop an algorithm capable of identifying the formulas introduced by \cite{voropaev2012number} within the $\WL 3$ CFG.

Given that CFG sentence generation corresponds to a tree structure, Monte Carlo Tree Search (MCTS) is a natural fit for this problem. Furthermore, we show that transformer architectures can be modeled as Pushdown Automata (PDAs), which are equivalent to CFGs. Thus, we employ transformers to learn the policy and value functions within a MCTS-based Reinforcement Learning (RL) algorithm \citep{zhang1995reinforcement,silver2018general,hubert2021learning,fawzi2022discovering}. We introduce Grammar Reinforcement Learning (GRL), an algorithm designed to search within a given grammar with the assistance of transformers.

%\cite{fawzi2022discovering}
%\begin{figure}
%    \centering
%    \includegraphics[width=0.3\textwidth]{image/discretespace.png}
%    \caption{Part of the discrete space of the $\WL 3$ CFG}
%    \label{fig:discrete}
%\end{figure}


%In this paper, we employ GRL algorithm to learn explicit formulas for substructure counting at the edge level in graphs. We apply our framework to the proposed $\WL 3$ CFG to construct the neural network used in the RL algorithm's learning phase. The primary objective of this experiment is to determine whether the resulting neural network can assist the RL algorithm in rediscovering the formulas proposed by \cite{voropaev2012number}. Remarkably, our model identified more efficient formulas for nearly all substructures, leading to calculation time improvements ranging from two- to six-fold.

The key contributions of this paper are as follows: (i) We present novel explicit formulas for substructure counting at the edge level in graphs, leading to substantial improvements in computational efficiency by factors of two to six. (ii) We introduce a framework that autonomously generates transformers capable of producing sentences within a specified CFG, demonstrating that autoregressive transformers can effectively model Pushdown Automata (PDAs). (iii) Leveraging this framework, we propose GRL, a RL algorithm designed to explore and search within a given grammar, with transformers playing a central role in guiding the search process.

The structure of this paper is as follows. Section \ref{sec: 2} focuses on substructure counting and Context-Free Grammars (CFGs), providing their definition and introducing the $\WL 3$ CFG used in our RL algorithm. In Section \ref{sec: 3}, we demonstrate the link between transformers and CFGs through our proposed framework. Section \ref{sec: 4} details the RL algorithm employed in this study and its results on the substructure counting. Section \ref{sec: 5} addresses GRL limitations. Finally, the paper concludes with a summary of our findings and contributions, and suggests potential avenues for future research.

==> section/section1old.tex <==
\section{Introduction}\label{sec: 1}

In usual machine learning optimization problems, a model $f_\theta$ is parametrized by $\theta$ and maps input data $x$ from a dataset $\cur D$ to a space $\R^d$. The goal is to find the parameters $\theta$ that minimize a loss function $\cur L$, which measures the discrepancy between the model's prediction $f_\theta(x)$ and the true value $y_x$ for data $x \in \cur D$. This can be generalized by considering a family of functions $\cur F$, where each function $f \in \cur F$ maps data $x$ from $\cur D$ to $\R^d$. The objective is to find the best function $f\in \cur F$ that minimizes the loss function $\cur L$ across the data $\cur D$. We propose to show that this general problem can be resolve with machine learning.

Graph Neural Networks (GNNs) have been extensively studied for their ability to process and analyze graph-structured data. However, despite their success, Message Passing Neural Networks (MPNNs) \cite{kipf2016semi,xu2018powerful} are limited in their expressive power, constrained  by the first-order Weisfeiler-Lehman ($\WL 1$) test, a well-known method in graph theory used for graph isomorphism testing. To address these limitations, novel models has been proposed that surpass $\WL 1$ expressiveness. Some models emulate the $\WL 3$ test, which involves higher-dimensional color refinements and provides enhanced discriminative power for graph isomorphism tasks \cite{morris2019wl,maron2018invariant,maron2019provably}. Additionally, strategies have been introduced to apply GNNs on subgraphs constructed by specific policies, thereby capturing more intricate structural patterns in the graph \cite{bevilacqua2021equivariant,frasca2022understanding,huang2022boosting}. Other models enhance expressiveness by incorporating subgraph counting mechanisms, which allow the network to recognize and leverage the presence of various subgraph structures \cite{huang2021short,bouritsas2022improving}. Furthermore, techniques from language theory have been employed to improve the expressive power of GNNs, utilizing formal grammatical structures to encode and process graph data more effectively \cite{balcilarexpresspower,piquenot2024grammatical}.

Nonetheless, any model is ultimately bounded by some $\WL k$ for a sufficiently large $k$. The WL hierarchy defines explicit families of functions suitable for our general problem framework.  Practically, \cite{matlang} introduced MATLANG a matrix language and \cite{geerts2021expressiveness} linked the subset of operation $\cur L_3 = \{ \cdot, \transpose \ , \diag , \onevector , \odot  \}$ and $\WL 3$ by showing that sentences in $\ML(\cur L_3)$ applied to adjacency matrices separate the same pairs of graphs than $\WL 3$. This paper focuses on $\cur F_{\cur L_3}$, defined as the set of sentences of $\ML{\cur L_3}$.


To generate sentences, and thus functions in $\cur F_{\cur L_3}$, recent research has proposed using Context-Free Grammar (CFG) \cite{piquenot2024grammatical}. We demonstrate that the $\WL3$ CFG proposed by \cite{piquenot2024grammatical} can be reduced while maintaining its expressive power. Sentences in such CFG form a discrete space where conventional gradient-based algorithms are unsuitable, as illustrated in Figure \ref{fig:discrete}. \cite{fawzi2022discovering} discovered improved matrix multiplication using a Monte Carlo Tree Search (MCTS) based Reinforcement Learning (RL) algorithm. Since CFG sentence production corresponds to a tree, MCTS is a natural fit. We show that transformer architectures can be modeled as PushDown Automata (PDAs), equivalent to CFGs. Thus, we can use transformers to learn the policy and value functions in the MCTS-based RL algorithm. We propose Grammar Reinforcement Learning (GRL), an algorithm that searches within a given grammar assisted by transformers.



\begin{figure}
    \centering
    \includegraphics[width=0.3\textwidth]{image/discretespace.png}
    \caption{Part of the discrete space of the $\WL 3$ CFG}
    \label{fig:discrete}
\end{figure}



The counting power of $\WL 3$ at graph and node levels has been studied by \cite{furer2017combinatorial,arvind2020weisfeiler}. Independently of WL, \cite{voropaev2012number} proposed explicit matrix formulas to count paths up to length six at the edge level in graphs. 

In this paper, we employ GRL algorithm to learn explicit formulas for substructure counting at the edge level in graphs. We apply our framework to the proposed $\WL 3$ CFG to build the neural network for the RL algorithm's learning phase. The primary objective of this experiment is to determine if the resulting neural network can assist the RL algorithm in discovering the formulas proposed by \cite{voropaev2012number}. Surprisingly, the model identified more efficient formulas for nearly all substructures, improving calculation times by factors of two to six.

The key contributions of this paper are summarized as follows. We demonstrate that the $\WL 3$ CFG proposed by \cite{piquenot2024grammatical} can be reduced while retaining its expressive power. we also propose a framework that automatically generates transformers capable of producing sentences in a specified CFG, showcasing the ability of autoregressive transformers to model Pushdown Automata (PDAs). Using our proposed framework within a Reinforcement Learning (RL) algorithm, we learn new explicit formulas for substructure counting at the edge level in graphs, significantly improving calculation times by factors of two to six.

The structure of this paper is as follows. Section \ref{sec: 2} focuses on Context-Free Grammars (CFGs), providing their definition and introducing $\WL 3$ CFG. In Section \ref{sec: 3}, we demonstrate the link between transformers and CFGs through our proposed framework. Section \ref{sec: 4} addresses substructure counting and details the RL algorithm employed in this study. Section \ref{sec: 5} addresses GLR limitations. Finally, the paper concludes with a summary of our findings and contributions, and suggests potential avenues for future research.


